Decentralized Online Learning in Task Assignment Games for Mobile Crowdsensing

The problem of coordinated data collection is studied for a mobile crowdsensing (MCS) system. A mobile crowdsensing platform (MCSP) sequentially publishes sensing tasks to the available mobile units (MUs) that signal their willingness to participate in a task by sending sensing offers back to the MCSP. From the received offers, the MCSP decides the task assignment. A stable task assignment must address two challenges: the MCSP's and MUs' conflicting goals, and the uncertainty about the MUs' required efforts and preferences. To overcome these challenges a novel decentralized approach combining matching theory and online learning, called collision-avoidance multi-armed bandit with strategic free sensing (CA-MAB-SFS), is proposed. The task assignment problem is modeled as a matching game considering the MCSP's and MUs' individual goals while the MUs learn their efforts online. Our innovative "free-sensing" mechanism significantly improves the MU's learning process while reducing collisions during task allocation. The stable regret of CA-MAB-SFS, i.e., the loss of learning, is analytically shown to be bounded by a sublinear function, ensuring the convergence to a stable optimal solution. Simulation results show that CA-MAB-SFS increases the MUs' and the MCSP's satisfaction compared to state-of-the-art methods while reducing the average task completion time by at least 16%.

==> algorithms/gs.tex <==
\begin{algorithm}[t]
\scriptsize
\caption{Offline Deferred Acceptance}\label{alg:cap}
\begin{algorithmic}[1]
\Require initalize all tasks and users as unassigned
\While {a free user $m$ exists and has not porposed to every task}
    \State $w$ = task with highest reward the user has not yet proposed
    \If{$w$-th task has no user assigned}
        \State the user $m$ is assigned to the $w$-th task
    \Else
        \If{$w$-th task prefers the user $m$ to assigned user $m'$}
            \State $m'$ becomes unassigned
            \State $m$ is assigned to $w$
        \EndIf
    \EndIf
\EndWhile
\State $\Bar{A}^{(k)} \xleftarrow[]{} A^{(k)}$
\end{algorithmic}
\end{algorithm}

==> algorithms/ouralgo.tex <==
\begin{algorithm}[t]
 \scriptsize
\caption{CA-MAB-FS}\label{alg:cap}
\begin{algorithmic}[1]
\REQUIRE $\lambda \in [0,1) , \hat{Q}_{k,0}(n) = 0 , \hat{J}_{k,0}(n) = 0$
\For{$t = 1,\dots,T$}
    \For{$k = 1,\dots,N$}
            \If{$t = 1$}
                \State \text{Sample a MCSP $\taskWithIndex{n} \in \setOfTasks$ uniformly at random.} \State \text{Set $A_t^{(k)} \gets a_n$}
            \Else
                \State Draw $D^{(k)}(t) \sim Ber(\lambda)$ independently
                %\State $N \gets n$
                \If{$D^{(k)}(t) = 0$}
                    %\If{$k$-th user was deferred often at task $n$}
                    %\If{if $k$-th MU was deferred %multiple times at MCSP $n$}
                    %    \State set $P_{k,n,t} \xleftarrow[]{} 0$ \algorithmiccomment{free-sensing}
                    %    \Else
                    %    \State determine bids $P_{k,n,t}$ based on learned rewards
                    %\EndIf
                    
                    % determine set of bids:
                    %\[
                    \State $P_{k,n,t}$= 
                    \begin{cases}
                        0,& \text{if } \gamma_{k,j,t} = 1\\
                        f(\hat{J}_{k,t-1}(n)),              & \text{otherwise}
                    \end{cases}
                    %\]
                     
                    \State transmit bids $P_{k,n,t}$ to each MCSP
                    \State receive binary feedback and update plausible set $S^{(k)}(t)$ for \MUwithIndex{k}:
                    \State $S^{(k)} := \{a_j: w_{i,j} - P_{i,j,t} >_{a_j} w_{k,j} - P_{k,j,t} \; \text{or} \;$
                    \STATEx $\MUwithIndex{i} = \MUwithIndex{k}, \; \text{where} \; \Bar{A}^{(k)}(t-1) = a_j \}$

                    \State choose $\taskWithIndex{n}\in S^{(k)}(t)$ using $\epsilon$ - greedy and place bid. Set
                    $A^{(i)}_t \xleftarrow[]{} \taskWithIndex{n}$
                \Else
                    \State place bid for $A^{(k)}_{t-1}$. Set $A^{(k)}_t \xleftarrow[]{} A^{(k)}_{t-1}$
                \EndIf 
            \EndIf %\taskWithIndex{A^{(k)}_t}
            \If{$a_{A^{(k)}_t}$ chooses $\MUwithIndex{k}$}
                \State sense $U^{MU}_{k,n,t}$ and $\totalTime$
                \State
                $\hat{Q}_{k,t}(n) \xleftarrow[]{}  \alpha^t \cdot U^{MU}_{k,n,t} + (1-\alpha^t) \cdot \hat{Q}_{k,t-1}(n)$
                \State
                $\hat{J}_{k,t}(n) \xleftarrow[]{}  \alpha^t \cdot \totalTime + (1-\alpha^t) \cdot \hat{J}_{k,t-1}(n)$
                \State $\Bar{A}^{(k)}(t) = a_{A^{(k)}_t}$
            \Else
                \State $\Bar{A}^{(k)}(t) = \varnothing$ , $\hat{Q}_{k,t}(n) \xleftarrow[]{}  \hat{Q}_{k,t-1}(n)$
                , $\hat{J}_{k,t}(n) \xleftarrow[]{}  \hat{J}_{k,t-1}(n)$
            \EndIf
    \EndFor  
\EndFor
\end{algorithmic}
\end{algorithm}


==> tables/evaluation_parameters.tex <==
	 \centering{
	 	\def\arraystretch{1.2}
	\begin{tabular}{|c|l|}
	\hline
	Parameter & Value  \\
	\hline
	Number of MUs & $ K = 200$ \\
	Payment function $f$ & Linear \\
	                     & $f(\totalTime,\totalEnergy) = \beta \cdot \totalTime$ \\
	Energy sensitivity & $\energySensitivity$ \\
	\hline
	Bandwidth $b_{m}$ per resource block & $\SI{200}{\kilo\hertz}$ \\
	Noise power $\sigma^2$ & $10^{-13}\,\SI{}{\watt}$ \\
	Transmit power $p_k$ of $\MUk$ & $\SI{200}{\milli\watt}$ \\
	Sensor power $p_k$ of $\MUk$ & $\SI{200}{\milli\watt}$ \\
	Channel gain $|h_{k,m}|^2$ & $\sim d^{-3}$ (Urban scenario)\\
	\hline
	Number of sensing tasks &   $N = 4$ \\
	Size $s_n$ of the sensing task result & Small: \SI{300}{\kilo\bit} \\
	                                      & Large: \SI{600}{\kilo\bit}\\
	Deadline $\deadlineOfTask$ of the sensing task & \SI{100}{\milli\second} \\
	\hline
	Exploration parameter $\epsilon_t$ & \\
	Collision-Avoidance parameter $\lambda$ & 0.1\\
	Free-exploration parameter $\lambda$ & 0.1\\
	\hline
	\end{tabular}}

==> tables/large_equation.tex <==
\begin{figure*}[!t]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
\setcounter{equation}{5}
\begin{align}
\label{eqn_dbl_x}
 R_k(T) & \leq \Delta_k  \sum_{t=1}^T \mathbb{P}(\mathbf{x}_t\notin{}X^{\mathrm{stable}}) \leq \Delta_k \sum_{t=1}^T  \mathbb{P}(E_{1,t}) + \mathbb{P}(\bar{E}_{1,t}) \cdot \mathbb{P}( E_{2,t}) \biggr)\\
& \leq \Delta_k  \biggl( \underbrace{K\frac{N-1}{N} (\log(T) + 1)}_{\text{Appendix 1}} + \sum_{t=1}^T\underbrace{\mathbb{P}(\bar{E}_{1,t})}_{\leq 1} \mathbb{P}( E_{2,t}) \biggr) \\
& \leq \Delta_k  \biggl( K\frac{N-1}{N} (\log(T) + 1) + \underbrace{ \frac{2N^5K^2}{\rho^{N^4+1}} \log(T)  \biggl( \biggl( { \color{red} TODO: \sum_{t=1}^T  \mathbb{P} ( \hat{Q}_{k,t}(i) > \hat{Q}_{k,t}(j) )  } \biggr)  + 6+ \frac{N^4}{\rho^{N^4}} \biggr)}_{\text{Appendix 2}}\biggr)
%& \leq \Delta_k  \biggl( K\frac{N-1}{N} (\log(T) + 1) + \frac{2N^5K^2}{\rho^{N^4+1}} \log(T) \biggl(\log(T) + \frac{1}{T}+ \frac{2}{\Delta_k^2}\frac{1}{T}e^{\frac{\Delta_k}{2T}} \biggr)  + 6+ \frac{N^4}{\rho^{N^4}} \biggr)
\end{align}
% Restore the current equation number.
%\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}
